Measuring Ethics in AI with AI: A Methodology and Dataset Construction

Recently, the use of sound measures and metrics in Artificial Intelligence has become the subject of interest of academia, government, and industry. Efforts towards measuring different phenomena have gained traction in the AI community, as illustrated by the publication of several influential field reports and policy documents. These metrics are designed to help decision takers to inform themselves about the fast-moving and impacting influences of key advances in Artificial Intelligence in general and Machine Learning in particular. In this paper we propose to use such newfound capabilities of AI technologies to augment our AI measuring capabilities. We do so by training a model to classify publications related to ethical issues and concerns. In our methodology we use an expert, manually curated dataset as the training set and then evaluate a large set of research papers. Finally, we highlight the implications of AI metrics, in particular their contribution towards developing trustful and fair AI-based tools and technologies. Keywords: AI Ethics; AI Fairness; AI Measurement. Ethics in Computer Science.

==> Measuring Ethics in Ai with AI [Arxiv 2021]/tabs/both.tex <==
\begin{table}[hptb]
    \tiny
    \centering
    \begin{tabular}{ccccccccccccc}
    \toprule
        \multirow{2}{*}{Year} & \multicolumn{6}{c}{Conferences} & \multicolumn{6}{c}{Journals} \\
         & AAAI & ICML & ICRA & IJCAI & IROS & NeuRIPS & CACM & Computer & Trans. & Trans. AI & Trans. Robotics & JAIR \\
    \midrule
% 1969 & - & - & - & 0.048 & - & - \\
% 1971 & - & - & - & 0.046 & - & - \\
% 1973 & - & - & - & 0.071 & - & - & - & 0.038 & 0.004 & - & - & - \\
% 1974 & - & - & - & - & - & - & - & 0.000 & 0.010 & - & - & - \\
% 1975 & - & - & - & 0.061 & - & - & 0.000 & 0.011 & 0.012 & - & - & - \\
% 1976 & - & - & - & 0.061 & - & - & 0.000 & 0.000 & 0.008 & - & - & - \\
% 1977 & - & - & - & 0.068 & - & - & 0.000 & 0.009 & 0.008 & - & - & - \\
% 1978 & - & - & - & - & - & - & 0.000 & 0.000 & 0.004 & - & - & - \\
% 1979 & - & - & - & 0.018 & - & - & 0.000 & 0.011 & 0.008 & - & - & - \\
1980 & 0.043 & - & - & - & - & - & 0.000 & 0.000 & 0.002 & - & - & - \\
1981 & - & - & - & 0.037 & - & - & 0.000 & 0.010 & 0.008 & - & - & - \\
1982 & 0.010 & - & - & - & - & - & 0.000 & 0.021 & 0.003 & - & - & - \\
1983 & 0.011 & - & - & 0.041 & - & - & 0.007 & 0.009 & 0.003 & - & - & - \\
1984 & 0.029 & - & 0.014 & - & - & - & 0.000 & 0.025 & 0.003 & - & - & - \\
1985 & - & - & 0.012 & 0.050 & - & - & 0.007 & 0.021 & 0.007 & - & - & - \\
1986 & 0.035 & - & 0.015 & - & - & - & 0.000 & 0.023 & 0.010 & - & - & - \\
1987 & 0.014 & - & 0.015 & 0.033 & - & 0.000 & 0.000 & 0.052 & 0.006 & - & - & - \\
1988 & 0.020 & - & 0.006 & - & - & 0.000 & 0.008 & 0.000 & 0.003 & - & - & - \\
1989 & - & - & 0.000 & 0.015 & 0.023 & 0.010 & 0.000 & 0.030 & 0.009 & - & 0.000 & - \\
1990 & 0.040 & - & 0.003 & - & 0.029 & 0.000 & 0.000 & 0.012 & 0.004 & 0.000 & 0.000 & - \\
1991 & 0.000 & - & 0.005 & 0.047 & 0.004 & 0.007 & 0.000 & 0.000 & 0.004 & 0.000 & 0.010 & - \\
1992 & 0.038 & - & 0.007 & - & 0.003 & 0.008 & 0.013 & 0.023 & 0.003 & 0.000 & 0.000 & - \\
1993 & 0.015 & 0.000 & - & 0.046 & 0.010 & 0.006 & 0.000 & 0.013 & 0.003 & 0.000 & 0.000 & 0.000 \\
1994 & 0.020 & 0.044 & 0.011 & - & 0.011 & 0.007 & 0.008 & 0.011 & 0.003 & 0.008 & 0.014 & 0.071 \\
1995 & - & 0.029 & 0.024 & 0.023 & - & 0.000 & 0.008 & 0.006 & 0.003 & 0.000 & 0.000 & 0.037 \\
1996 & - & 0.015 & 0.009 & - & 0.013 & 0.007 & 0.012 & 0.023 & 0.002 & 0.005 & 0.011 & 0.000 \\
1997 & - & 0.021 & 0.007 & 0.036 & 0.014 & 0.006 & 0.008 & 0.023 & 0.002 & 0.000 & 0.000 & 0.000 \\
1998 & - & 0.000 & 0.002 & - & 0.013 & 0.020 & 0.008 & 0.017 & 0.002 & 0.000 & 0.010 & 0.000 \\
1999 & - & 0.019 & 0.012 & 0.010 & 0.010 & 0.007 & 0.004 & 0.017 & 0.002 & 0.000 & 0.002 & 0.000 \\
2000 & 0.250 & 0.007 & 0.003 & - & 0.016 & 0.007 & 0.007 & 0.020 & 0.004 & 0.004 & 0.002 & 0.000 \\
2001 & - & 0.013 & 0.006 & 0.010 & 0.003 & 0.010 & 0.004 & 0.006 & 0.003 & 0.004 & 0.005 & 0.040 \\
2002 & - & 0.000 & 0.004 & - & 0.022 & 0.010 & 0.005 & 0.023 & 0.004 & 0.000 & 0.002 & 0.000 \\
2003 & - & 0.009 & 0.016 & 0.014 & 0.013 & 0.015 & 0.009 & 0.027 & 0.003 & 0.000 & 0.007 & 0.000 \\
2004 & 0.031 & 0.017 & 0.024 & - & 0.012 & 0.015 & 0.004 & 0.033 & 0.005 & 0.004 & 0.002 & 0.000 \\
2005 & 0.009 & 0.000 & 0.014 & 0.017 & 0.012 & 0.005 & 0.010 & 0.035 & 0.003 & 0.000 & 0.002 & 0.026 \\
2006 & 0.031 & 0.000 & 0.007 & - & 0.011 & 0.005 & 0.002 & 0.036 & 0.003 & 0.000 & 0.005 & 0.023 \\
2007 & 0.008 & 0.000 & 0.009 & 0.006 & 0.009 & 0.009 & 0.007 & 0.011 & 0.006 & 0.004 & 0.010 & 0.000 \\
2008 & 0.023 & 0.000 & 0.014 & - & 0.010 & 0.012 & 0.006 & 0.024 & 0.006 & 0.002 & 0.010 & 0.017 \\
2009 & - & 0.000 & 0.008 & 0.000 & 0.012 & 0.008 & 0.008 & 0.013 & 0.005 & 0.008 & 0.007 & 0.000 \\
2010 & 0.010 & 0.006 & 0.007 & - & 0.013 & 0.000 & 0.005 & 0.034 & 0.004 & 0.003 & 0.005 & 0.000 \\
2011 & 0.019 & 0.000 & 0.008 & 0.016 & 0.011 & 0.010 & 0.005 & 0.020 & 0.007 & 0.003 & 0.006 & 0.000 \\
2012 & 0.026 & 0.000 & 0.014 & - & 0.013 & 0.005 & 0.010 & 0.020 & 0.004 & 0.010 & 0.005 & 0.000 \\
2013 & 0.012 & - & 0.012 & 0.016 & 0.011 & 0.008 & 0.008 & 0.038 & 0.005 & 0.003 & 0.003 & 0.033 \\
2014 & 0.028 & 0.003 & 0.010 & - & 0.011 & 0.005 & 0.008 & 0.014 & 0.007 & 0.002 & 0.002 & 0.030 \\
2015 & 0.021 & 0.000 & 0.008 & 0.009 & 0.017 & 0.005 & 0.011 & 0.026 & 0.004 & 0.016 & 0.003 & 0.000 \\
2016 & 0.031 & 0.003 & 0.012 & 0.026 & 0.015 & 0.005 & 0.007 & 0.025 & 0.006 & 0.015 & 0.001 & 0.000 \\
2017 & 0.030 & 0.007 & 0.011 & 0.028 & 0.008 & 0.016 & 0.006 & 0.039 & 0.006 & 0.015 & 0.003 & 0.015 \\
% 2018 & 0.034 & 0.026 & 0.010 & 0.041 & 0.015 & - & 0.008 & 0.054 & 0.007 & 0.005 & 0.006 & 0.043 \\
% 2019 & - & 0.029 & - & - & - & - & 0.002 & 0.018 & 0.006 & 0.012 & 0.003 & 0.185 \\
    \bottomrule
    \end{tabular}
    \caption{Ratio of papers that were considered by the model to be ethics-related on the four AI and two Robotics conferences, and six journals. Respectively AAAI, ICML, ICRA, IJCAI, IROS, NeurIPS, Communications of the ACM, IEEE Computer, IEEE Transactions, IEEE Transactions (AI), IEEE Transactions on Robotics, and Journal of Artificial Intelligence Research.}
    \label{tab:conferences}
\end{table}

==> Measuring Ethics in Ai with AI [Arxiv 2021]/tabs/conferences.tex <==
\begin{table}[hptb]
    \small
    \centering
    \begin{tabular}{ccccccc}
    \toprule
        Year & AAAI & ICML & ICRA & IJCAI & IROS & NeurIPS\\
    \midrule
% 1969 & - & - & - & 0.048 & - & -\\
% 1971 & - & - & - & 0.046 & - & -\\
% 1973 & - & - & - & 0.071 & - & -\\
% 1975 & - & - & - & 0.061 & - & -\\
% 1977 & - & - & - & 0.068 & - & -\\
% 1979 & - & - & - & 0.018 & - & -\\
1980 & 0.043 & - & - & - & - & -\\
1981 & - & - & - & 0.037 & - & -\\
1982 & 0.010 & - & - & - & - & -\\
1983 & 0.011 & - & - & 0.041 & - & -\\
1984 & 0.029 & - & 0.014 & - & - & -\\
1985 & - & - & 0.012 & 0.050 & - & -\\
1986 & 0.035 & - & 0.015 & - & - & -\\
1987 & 0.014 & - & 0.015 & 0.033 & - & 0.000\\
1988 & 0.020 & - & 0.006 & - & - & 0.000\\
1989 & - & - & 0.000 & 0.015 & 0.023 & 0.010\\
1990 & 0.040 & - & 0.003 & - & 0.029 & 0.000\\
1991 & 0.000 & - & 0.005 & 0.047 & 0.004 & 0.007\\
1992 & 0.038 & - & 0.007 & - & 0.003 & 0.008\\
1993 & 0.015 & 0.000 & - & 0.046 & 0.010 & 0.006\\
1994 & 0.020 & 0.044 & 0.011 & - & 0.011 & 0.007\\
1995 & - & 0.029 & 0.024 & 0.023 & - & 0.000\\
1996 & - & 0.015 & 0.009 & - & 0.013 & 0.007\\
1997 & - & 0.021 & 0.007 & 0.036 & 0.014 & 0.006\\
1998 & - & 0.000 & 0.002 & - & 0.013 & 0.020\\
1999 & - & 0.019 & 0.012 & 0.010 & 0.010 & 0.007\\
2000 & 0.250 & 0.007 & 0.003 & - & 0.016 & 0.007\\
2001 & - & 0.013 & 0.006 & 0.010 & 0.003 & 0.010\\
2002 & - & 0.000 & 0.004 & - & 0.022 & 0.010\\
2003 & - & 0.009 & 0.016 & 0.014 & 0.013 & 0.015\\
2004 & 0.031 & 0.017 & 0.024 & - & 0.012 & 0.015\\
2005 & 0.009 & 0.000 & 0.014 & 0.017 & 0.012 & 0.005\\
2006 & 0.031 & 0.000 & 0.007 & - & 0.011 & 0.005\\
2007 & 0.008 & 0.000 & 0.009 & 0.006 & 0.009 & 0.009\\
2008 & 0.023 & 0.000 & 0.014 & - & 0.010 & 0.012\\
2009 & - & 0.000 & 0.008 & 0.000 & 0.012 & 0.008\\
2010 & 0.010 & 0.006 & 0.007 & - & 0.013 & 0.000\\
2011 & 0.019 & 0.000 & 0.008 & 0.016 & 0.011 & 0.010\\
2012 & 0.026 & 0.000 & 0.014 & - & 0.013 & 0.005\\
2013 & 0.012 & - & 0.012 & 0.016 & 0.011 & 0.008\\
2014 & 0.028 & 0.003 & 0.010 & - & 0.011 & 0.005\\
2015 & 0.021 & 0.000 & 0.008 & 0.009 & 0.017 & 0.005\\
2016 & 0.031 & 0.003 & 0.012 & 0.026 & 0.015 & 0.005\\
2017 & 0.030 & 0.007 & 0.011 & 0.028 & 0.008 & 0.016\\
% 2018 & 0.034 & 0.026 & 0.010 & 0.041 & 0.015 & -\\
% 2019 & - & 0.029 & - & - & - & -\\
    \bottomrule
    \end{tabular}
    \caption{Ratio of papers that were considered by the model to be ethics-related topic on the four AI and two Robotics conferences.}
    \label{tab:conferences}
\end{table}

==> Measuring Ethics in Ai with AI [Arxiv 2021]/tabs/hyperparams.tex <==
\begin{table}[hptb]
    \small
    \centering
    \begin{tabular}{ccc}
    \toprule
        Model & Hyperparameter & Options \\
    \midrule
        \multirow{2}{*}{LR}         & Inv. Reg. Strength       & 0.25, 0.5, 1, 2, 4 \\ 
                                    & Regularisation           & $l1$, $l2$ \\ \midrule
        \multirow{2}{*}{AB}   & Num. of Estimators       & 8, 32, 128, 512 \\ 
                                    & Learning Rate            & 0.125, 0.25, 0.5, 1 \\ \midrule
        \multirow{2}{*}{GB}  & Num. of Estimators       & 8, 32, 128, 512 \\
                                    & Max. Tree Depth          & 1, 2 , 4, 8 \\ \midrule
        \multirow{2}{*}{RF}         & Num. of Estimators       & 8, 32, 128, 512 \\
                                    & Max. Tree Depth          & 1, 2 , 4, 8 \\ \midrule
        \multirow{3}{*}{DT}         & Optimisation Criterion   & Gini, Entropy \\
                                    & Splitting Method         & Best, Random \\
                                    & Max. Tree Depth          & 1, 2 , 4, 8 \\
        \multirow{4}{*}{MLP}        & Activation function      & TanH, ReLU \\ \midrule
                                    & Learning Rate            & $10^{-3}$, $10^{-4}$, $10^{-5}$ \\
                                    & Learning Rate Technique  & Adaptative, Constant \\
                                    & Max. Training Iterations & 32, 128, 512 \\
    \bottomrule
    \end{tabular}
    \caption{Models and Hyperparameters used in the experiments. LR stands for Logistic Regression, AB for Adaptive Boosting, GB for Gradient Boosting, RF for Random Forest, DT for Decision Tree, MLP for Multilayer Perceptron. For the MLP model we used the Adam optimiser.}
    \label{tab:hyperparams}
\end{table}

==> Measuring Ethics in Ai with AI [Arxiv 2021]/tabs/journals.tex <==
\begin{table}[hptb]
    \small
    \centering
    \begin{tabular}{ccccccc}
    \toprule
        Year & CACM & C  & T. & TAI & TR & JAIR\\
    \midrule
    % 1963 & - & - & 0.005 & - & - & -\\
    % 1964 & - & - & 0.000 & - & - & -\\
    % 1965 & - & - & 0.003 & - & - & -\\
    % 1966 & - & - & 0.000 & - & - & -\\
    % 1967 & - & - & 0.000 & - & - & -\\
    % 1968 & - & - & 0.005 & - & - & -\\
    % 1969 & - & - & 0.008 & - & - & -\\
    % 1970 & - & 0.000 & 0.004 & - & - & -\\
    % 1971 & - & 0.038 & 0.002 & - & - & -\\
    % 1972 & - & 0.000 & 0.002 & - & - & -\\
    % 1973 & - & 0.038 & 0.004 & - & - & -\\
    % 1974 & - & 0.000 & 0.010 & - & - & -\\
    % 1975 & 0.000 & 0.011 & 0.012 & - & - & -\\
    % 1976 & 0.000 & 0.000 & 0.008 & - & - & -\\
    % 1977 & 0.000 & 0.009 & 0.008 & - & - & -\\
    % 1978 & 0.000 & 0.000 & 0.004 & - & - & -\\
    % 1979 & 0.000 & 0.011 & 0.008 & - & - & -\\
    1980 & 0.000 & 0.000 & 0.002 & - & - & -\\
    1981 & 0.000 & 0.010 & 0.008 & - & - & -\\
    1982 & 0.000 & 0.021 & 0.003 & - & - & -\\
    1983 & 0.007 & 0.009 & 0.003 & - & - & -\\
    1984 & 0.000 & 0.025 & 0.003 & - & - & -\\
    1985 & 0.007 & 0.021 & 0.007 & - & - & -\\
    1986 & 0.000 & 0.023 & 0.010 & - & - & -\\
    1987 & 0.000 & 0.052 & 0.006 & - & - & -\\
    1988 & 0.008 & 0.000 & 0.003 & - & - & -\\
    1989 & 0.000 & 0.030 & 0.009 & - & 0.000 & -\\
    1990 & 0.000 & 0.012 & 0.004 & 0.000 & 0.000 & -\\
    1991 & 0.000 & 0.000 & 0.004 & 0.000 & 0.010 & -\\
    1992 & 0.013 & 0.023 & 0.003 & 0.000 & 0.000 & -\\
    1993 & 0.000 & 0.013 & 0.003 & 0.000 & 0.000 & 0.000\\
    1994 & 0.008 & 0.011 & 0.003 & 0.008 & 0.014 & 0.071\\
    1995 & 0.008 & 0.006 & 0.003 & 0.000 & 0.000 & 0.037\\
    1996 & 0.012 & 0.023 & 0.002 & 0.005 & 0.011 & 0.000\\
    1997 & 0.008 & 0.023 & 0.002 & 0.000 & 0.000 & 0.000\\
    1998 & 0.008 & 0.017 & 0.002 & 0.000 & 0.010 & 0.000\\
    1999 & 0.004 & 0.017 & 0.002 & 0.000 & 0.002 & 0.000\\
    2000 & 0.007 & 0.020 & 0.004 & 0.004 & 0.002 & 0.000\\
    2001 & 0.004 & 0.006 & 0.003 & 0.004 & 0.005 & 0.040\\
    2002 & 0.005 & 0.023 & 0.004 & 0.000 & 0.002 & 0.000\\
    2003 & 0.009 & 0.027 & 0.003 & 0.000 & 0.007 & 0.000\\
    2004 & 0.004 & 0.033 & 0.005 & 0.004 & 0.002 & 0.000\\
    2005 & 0.010 & 0.035 & 0.003 & 0.000 & 0.002 & 0.026\\
    2006 & 0.002 & 0.036 & 0.003 & 0.000 & 0.005 & 0.023\\
    2007 & 0.007 & 0.011 & 0.006 & 0.004 & 0.010 & 0.000\\
    2008 & 0.006 & 0.024 & 0.006 & 0.002 & 0.010 & 0.017\\
    2009 & 0.008 & 0.013 & 0.005 & 0.008 & 0.007 & 0.000\\
    2010 & 0.005 & 0.034 & 0.004 & 0.003 & 0.005 & 0.000\\
    2011 & 0.005 & 0.020 & 0.007 & 0.003 & 0.006 & 0.000\\
    2012 & 0.010 & 0.020 & 0.004 & 0.010 & 0.005 & 0.000\\
    2013 & 0.008 & 0.038 & 0.005 & 0.003 & 0.003 & 0.033\\
    2014 & 0.008 & 0.014 & 0.007 & 0.002 & 0.002 & 0.030\\
    2015 & 0.011 & 0.026 & 0.004 & 0.016 & 0.003 & 0.000\\
    2016 & 0.007 & 0.025 & 0.006 & 0.015 & 0.001 & 0.000\\
    2017 & 0.006 & 0.039 & 0.006 & 0.015 & 0.003 & 0.015\\
    % 2018 & 0.008 & 0.054 & 0.007 & 0.005 & 0.006 & 0.043\\
    % 2019 & 0.002 & 0.018 & 0.006 & 0.012 & 0.003 & 0.185\\
    \bottomrule
    \end{tabular}
    \caption{Ratio of papers that were considered by the model to be on ethics-related topics on the analysed Journal Venues; respectively, [CACM] Communications of the ACM, [C] IEEE Computer, [T] IEEE Transactions, [TAI] IEEE Transactions (AI), [TR] IEEE Transactions on Robotics, and [JAIR] Journal of Artificial Intelligence Research.}
    \label{tab:journals}
\end{table}

==> tabs/both.tex <==
\begin{table}[hptb]
    \tiny
    \centering
    \begin{tabular}{ccccccccccccc}
    \toprule
        \multirow{2}{*}{Year} & \multicolumn{6}{c}{Conferences} & \multicolumn{6}{c}{Journals} \\
         & AAAI & ICML & ICRA & IJCAI & IROS & NeuRIPS & CACM & Computer & Trans. & Trans. AI & Trans. Robotics & JAIR \\
    \midrule
% 1969 & - & - & - & 0.048 & - & - \\
% 1971 & - & - & - & 0.046 & - & - \\
% 1973 & - & - & - & 0.071 & - & - & - & 0.038 & 0.004 & - & - & - \\
% 1974 & - & - & - & - & - & - & - & 0.000 & 0.010 & - & - & - \\
% 1975 & - & - & - & 0.061 & - & - & 0.000 & 0.011 & 0.012 & - & - & - \\
% 1976 & - & - & - & 0.061 & - & - & 0.000 & 0.000 & 0.008 & - & - & - \\
% 1977 & - & - & - & 0.068 & - & - & 0.000 & 0.009 & 0.008 & - & - & - \\
% 1978 & - & - & - & - & - & - & 0.000 & 0.000 & 0.004 & - & - & - \\
% 1979 & - & - & - & 0.018 & - & - & 0.000 & 0.011 & 0.008 & - & - & - \\
1980 & 0.043 & - & - & - & - & - & 0.000 & 0.000 & 0.002 & - & - & - \\
1981 & - & - & - & 0.037 & - & - & 0.000 & 0.010 & 0.008 & - & - & - \\
1982 & 0.010 & - & - & - & - & - & 0.000 & 0.021 & 0.003 & - & - & - \\
1983 & 0.011 & - & - & 0.041 & - & - & 0.007 & 0.009 & 0.003 & - & - & - \\
1984 & 0.029 & - & 0.014 & - & - & - & 0.000 & 0.025 & 0.003 & - & - & - \\
1985 & - & - & 0.012 & 0.050 & - & - & 0.007 & 0.021 & 0.007 & - & - & - \\
1986 & 0.035 & - & 0.015 & - & - & - & 0.000 & 0.023 & 0.010 & - & - & - \\
1987 & 0.014 & - & 0.015 & 0.033 & - & 0.000 & 0.000 & 0.052 & 0.006 & - & - & - \\
1988 & 0.020 & - & 0.006 & - & - & 0.000 & 0.008 & 0.000 & 0.003 & - & - & - \\
1989 & - & - & 0.000 & 0.015 & 0.023 & 0.010 & 0.000 & 0.030 & 0.009 & - & 0.000 & - \\
1990 & 0.040 & - & 0.003 & - & 0.029 & 0.000 & 0.000 & 0.012 & 0.004 & 0.000 & 0.000 & - \\
1991 & 0.000 & - & 0.005 & 0.047 & 0.004 & 0.007 & 0.000 & 0.000 & 0.004 & 0.000 & 0.010 & - \\
1992 & 0.038 & - & 0.007 & - & 0.003 & 0.008 & 0.013 & 0.023 & 0.003 & 0.000 & 0.000 & - \\
1993 & 0.015 & 0.000 & - & 0.046 & 0.010 & 0.006 & 0.000 & 0.013 & 0.003 & 0.000 & 0.000 & 0.000 \\
1994 & 0.020 & 0.044 & 0.011 & - & 0.011 & 0.007 & 0.008 & 0.011 & 0.003 & 0.008 & 0.014 & 0.071 \\
1995 & - & 0.029 & 0.024 & 0.023 & - & 0.000 & 0.008 & 0.006 & 0.003 & 0.000 & 0.000 & 0.037 \\
1996 & - & 0.015 & 0.009 & - & 0.013 & 0.007 & 0.012 & 0.023 & 0.002 & 0.005 & 0.011 & 0.000 \\
1997 & - & 0.021 & 0.007 & 0.036 & 0.014 & 0.006 & 0.008 & 0.023 & 0.002 & 0.000 & 0.000 & 0.000 \\
1998 & - & 0.000 & 0.002 & - & 0.013 & 0.020 & 0.008 & 0.017 & 0.002 & 0.000 & 0.010 & 0.000 \\
1999 & - & 0.019 & 0.012 & 0.010 & 0.010 & 0.007 & 0.004 & 0.017 & 0.002 & 0.000 & 0.002 & 0.000 \\
2000 & 0.250 & 0.007 & 0.003 & - & 0.016 & 0.007 & 0.007 & 0.020 & 0.004 & 0.004 & 0.002 & 0.000 \\
2001 & - & 0.013 & 0.006 & 0.010 & 0.003 & 0.010 & 0.004 & 0.006 & 0.003 & 0.004 & 0.005 & 0.040 \\
2002 & - & 0.000 & 0.004 & - & 0.022 & 0.010 & 0.005 & 0.023 & 0.004 & 0.000 & 0.002 & 0.000 \\
2003 & - & 0.009 & 0.016 & 0.014 & 0.013 & 0.015 & 0.009 & 0.027 & 0.003 & 0.000 & 0.007 & 0.000 \\
2004 & 0.031 & 0.017 & 0.024 & - & 0.012 & 0.015 & 0.004 & 0.033 & 0.005 & 0.004 & 0.002 & 0.000 \\
2005 & 0.009 & 0.000 & 0.014 & 0.017 & 0.012 & 0.005 & 0.010 & 0.035 & 0.003 & 0.000 & 0.002 & 0.026 \\
2006 & 0.031 & 0.000 & 0.007 & - & 0.011 & 0.005 & 0.002 & 0.036 & 0.003 & 0.000 & 0.005 & 0.023 \\
2007 & 0.008 & 0.000 & 0.009 & 0.006 & 0.009 & 0.009 & 0.007 & 0.011 & 0.006 & 0.004 & 0.010 & 0.000 \\
2008 & 0.023 & 0.000 & 0.014 & - & 0.010 & 0.012 & 0.006 & 0.024 & 0.006 & 0.002 & 0.010 & 0.017 \\
2009 & - & 0.000 & 0.008 & 0.000 & 0.012 & 0.008 & 0.008 & 0.013 & 0.005 & 0.008 & 0.007 & 0.000 \\
2010 & 0.010 & 0.006 & 0.007 & - & 0.013 & 0.000 & 0.005 & 0.034 & 0.004 & 0.003 & 0.005 & 0.000 \\
2011 & 0.019 & 0.000 & 0.008 & 0.016 & 0.011 & 0.010 & 0.005 & 0.020 & 0.007 & 0.003 & 0.006 & 0.000 \\
2012 & 0.026 & 0.000 & 0.014 & - & 0.013 & 0.005 & 0.010 & 0.020 & 0.004 & 0.010 & 0.005 & 0.000 \\
2013 & 0.012 & - & 0.012 & 0.016 & 0.011 & 0.008 & 0.008 & 0.038 & 0.005 & 0.003 & 0.003 & 0.033 \\
2014 & 0.028 & 0.003 & 0.010 & - & 0.011 & 0.005 & 0.008 & 0.014 & 0.007 & 0.002 & 0.002 & 0.030 \\
2015 & 0.021 & 0.000 & 0.008 & 0.009 & 0.017 & 0.005 & 0.011 & 0.026 & 0.004 & 0.016 & 0.003 & 0.000 \\
2016 & 0.031 & 0.003 & 0.012 & 0.026 & 0.015 & 0.005 & 0.007 & 0.025 & 0.006 & 0.015 & 0.001 & 0.000 \\
2017 & 0.030 & 0.007 & 0.011 & 0.028 & 0.008 & 0.016 & 0.006 & 0.039 & 0.006 & 0.015 & 0.003 & 0.015 \\
% 2018 & 0.034 & 0.026 & 0.010 & 0.041 & 0.015 & - & 0.008 & 0.054 & 0.007 & 0.005 & 0.006 & 0.043 \\
% 2019 & - & 0.029 & - & - & - & - & 0.002 & 0.018 & 0.006 & 0.012 & 0.003 & 0.185 \\
    \bottomrule
    \end{tabular}
    \caption{Ratio of papers that were considered by the model to be ethics-related on the four AI and two Robotics conferences, and six journals. Respectively AAAI, ICML, ICRA, IJCAI, IROS, NeurIPS, Communications of the ACM, IEEE Computer, IEEE Transactions, IEEE Transactions (AI), IEEE Transactions on Robotics, and Journal of Artificial Intelligence Research.}
    \label{tab:conferences}
\end{table}
